Unitary Synthesis of Clifford+T Circuits with Reinforcement Learning

This paper presents a deep reinforcement learning approach for synthesizing unitaries into quantum circuits. Unitary synthesis aims to identify a quantum circuit that represents a given unitary while minimizing circuit depth, total gate count, a specific gate count, or a combination of these factors. While past research has focused predominantly on continuous gate sets, synthesizing unitaries from the parameter-free Clifford+T gate set remains a challenge. Although the time complexity of this task will inevitably remain exponential in the number of qubits for general unitaries, reducing the runtime for simple problem instances still poses a significant challenge. In this study, we apply the tree-search method Gumbel AlphaZero to solve the problem for a subset of exactly synthesizable Clifford+T unitaries. Our method effectively synthesizes circuits for up to five qubits generated from randomized circuits with up to 60 gates, outperforming existing tools like QuantumCircuitOpt and MIN-T-SYNTH in terms of synthesis time for larger qubit counts. Furthermore, it surpasses Synthetiq in successfully synthesizing random, exactly synthesizable unitaries. These results establish a strong baseline for future unitary synthesis algorithms.

==> ApxDatastructure.tex <==
In the following, we describe our internal environment data structures.

TODO

\begin{algorithm}
\caption{Environment Data Structures.}
\label{alg:data-structures}
\begin{algorithmic}[1]
    \STATE \textbf{Data Structure} QuantumCircuit
    \STATE \quad $circuit \; layout$: List[List[List[integer]]]
    \STATE \quad $unitary$: List[List[complex]]
    \STATE \quad $operations \; forward \; commuting$: List[boolean]
    \STATE \quad $gate \; counts$: List[integer]
\end{algorithmic}

\label{alg:sturcture-envstate}
\begin{algorithmic}[1]
    \STATE \textbf{Data Structure} EnvironmentState
    \STATE \quad $time \; step$: integer
    \STATE \quad $circuit$: QuantumCircuit
    \STATE \quad $action \; history$: List[integer]
    \STATE \quad $target \; circuit$: QuantumCircuit
    \STATE \quad $target \; action \; history$: List[integer]
    \STATE \quad $fidelity$: float
    \STATE \quad $rng \; key$: integer
\end{algorithmic}
\end{algorithm}

==> ApxSolCirc.tex <==
Here, in  \cref{fig:2qubitfigs}, \cref{fig:3qubitfigs} we provide some known decompositions of specific and structured unitaries which also were 
the target for our RL agent in \cref{tab:SpecificUnitaries}. The decompositions are taken from 
\cite{amy2013meet} and \cite{mosca2021polynomial}. In  \cref{fig:4qubitfigs}, we provide the structure of the target 
4-qubit unitaries with the number of T gates found by our RL agent shown in \cref{tab:SpecificUnitaries}.
\begin{figure}
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \\
			& \gate{Y} &
		\end{quantikz}=\begin{quantikz}
			&  & \ctrl[verticalwire=c]{1}  &  & \\
			& \gate{P^{\dagger}} & \targ{} & \gate{P} &
		\end{quantikz}
		\caption{Decomposition of Controlled-Y Gate}
	\end{subfigure}%
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \\
			& \gate{Z} &
		\end{quantikz}=\begin{quantikz}
			&  & \ctrl[verticalwire=c]{1}  &  & \\
			& \gate{H} & \targ{} & \gate{H} &
		\end{quantikz}
		\caption{Decomposition of Controlled-Z Gate}
	\end{subfigure} \\
	\vskip -0.2in
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \\
			& \gate{H} &
		\end{quantikz}=\begin{quantikz}
			&  &  &  & \ctrl[verticalwire=c]{1} &  &  &  & \\
			& \gate{P} & \gate{H} & \gate{T} & \targ{} & \gate{T^{\dagger}} & \gate{H} & \gate{P^{\dagger}} &
		\end{quantikz}
		\caption{Decomposition of Controlled-H Gate}
	\end{subfigure} \\
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \\
			& \gate{P} &
		\end{quantikz}=\begin{quantikz}
			& \targ{}  & \gate{T^{\dagger}}  & \targ{}  & \gate{T}   & \\
			& \ctrl[verticalwire=c]{-1} &  & \ctrl[verticalwire=c]{-1} & \gate{T}  &
		\end{quantikz}
		\caption{Decomposition of Controlled-P Gate}
	\end{subfigure}%
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \\
			& \gate{V} &
		\end{quantikz}=\begin{quantikz}
			& \gate{T} & \targ{}  & \gate{T^{\dagger}}  & \targ{} &   & \\
			& \gate{H} & \ctrl[verticalwire=c]{-1} & \gate{T}  & \ctrl[verticalwire=c]{-1} & \gate{H}  &
		\end{quantikz}
		\caption{Decomposition of Controlled-V Gate}
	\end{subfigure} \\
	\begin{subfigure}{.4\columnwidth}
		\begin{quantikz}
			& \gate[2]{W} & \\
			& &
		\end{quantikz}=\begin{quantikz}
			& \ctrl[verticalwire=c]{1} & \gate{P} & \gate{H} & \ctrl[verticalwire=c]{1} & \gate{T}  & \ctrl[verticalwire=c]{1} &  \gate{H} & \ctrl[verticalwire=c]{1} &  &  \\
			& \targ{} & \gate{P} &  & \targ{} & \gate{T^{\dagger}} & \targ{} &  & \targ{} & \gate{P^{\dagger}}  &
		\end{quantikz}
		\caption{Decomposition of W Gate}
	\end{subfigure}
	\caption{2-Qubit gate true decomposition as shown in \cite{amy2013meet}}
	\label{fig:2qubitfigs}
\end{figure}

\begin{figure}
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{2} & \\
			& \ctrl{1} & \\
			& \targ{} &
		\end{quantikz}=\begin{quantikz}
			& \gate{T^{\dagger}} & \targ{} & \gate{T} & \targ{} & \gate{T^{\dagger}} & \targ{} & \gate{T} & \targ{} & \\
			& \gate{T^{\dagger}} & & \ctrl{1} & \ctrl{-1} & \ctrl{1}  &  &  & \ctrl{-1} & \\
			& \gate{H} & \ctrl{-2} & \targ{} & \gate{T} & \targ{} & \ctrl{-2} & \gate{T^{\dagger}} & \gate{H} &
		\end{quantikz}
		\caption{Toffoli gate decomposition}
	\end{subfigure} \\
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \octrl{2} & \\
			& \ctrl{1} & \\
			& \targ{} & 
		\end{quantikz}=\begin{quantikz}
			 & \gate{T} & \targ{} & \gate{T^{\dagger}} & \targ{} & \gate{T} &  & \targ{} & \gate{T^{\dagger}} & \targ{} & \\
			 & &  & \gate{T^{\dagger}} & \ctrl{-1} & \targ{} & \gate{T} &  & \targ{} & \ctrl{-1}  & \\
			 & \gate{H} & \ctrl{-2} & \gate{T^{\dagger}} &  & \ctrl{-1} &  & \ctrl{-2} & \ctrl{-1} & \gate{H} & \\
		\end{quantikz}
		\caption{Single negated toffoli decomposition}
	\end{subfigure} \\
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& & \octrl{2} & \\
			& & \octrl{1} & \\
			& \targ{} & \targ{} &  
		\end{quantikz}=\begin{quantikz}
			&  &  & \gate{T^{\dagger}} & \ctrl{1} & \targ{} &  & \gate{T} &  & \targ{} & \ctrl{1} &  \\
			& \gate{T^{\dagger}} & \targ{} & \gate{T} & \targ{} &  & \gate{T} & \targ{} & \gate{T^{\dagger}} &  & \targ{} & \\
			& \gate{H} & \ctrl{-1} & \gate{T^{\dagger}} & \gate{P^{\dagger}} & \ctrl{-2} &  & \ctrl{-1} &  & \ctrl{-2} & \gate{H} & 
		\end{quantikz}
		\caption{Quantum OR decomposition}
	\end{subfigure} \\
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{2} & \ctrl{1} & \\
			& \ctrl{1} & \targ{} & \\
			& \targ{} &  &  
		\end{quantikz}=\begin{quantikz}
			& \gate{T} &  &  & \ctrl{2} & \ctrl{1}  & \ctrl{2} &  &  &  &  &  \\
			& \gate{T} & \targ{} & \gate{T^{\dagger}} &  & \targ{} &  & \gate{T} &  & \targ{} & \gate{T^{\dagger}} & \\
			& \gate{H} & \ctrl{-1} &  & \targ{} & \gate{T^{\dagger}} & \targ{} &  & \gate{T} & \ctrl{-1} & \gate{H} & 
		\end{quantikz}
		\caption{Peres gate decomposition}
	\end{subfigure}
	\caption{3-Qubit circuits decomposition as shown in \cite{amy2013meet} and \cite{mosca2021polynomial}}
	\label{fig:3qubitfigs}
\end{figure}

\begin{figure}

	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{2} & \\
			& \ctrl{1} & \\
			& \targ{} & \\
			& &
		\end{quantikz}
		\caption{Toffoli with 1 Ancilla}
	\end{subfigure}%
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{2} & & \\
			& \ctrl{1} & \ctrl{2} & \\
			& \targ{} & \ctrl{1} & \\
			& & \targ{} &
		\end{quantikz}
		\caption{2 Toffoli ($U_1$)}
	\end{subfigure}%
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{2} & & \ctrl{2} & \\
			& \ctrl{1} & \ctrl{2} & \ctrl{1} & \\
			& \targ{} & \ctrl{1} & \targ{} & \\
			& & \targ{} &  &
		\end{quantikz}
		\caption{3 Toffoli ($U_2$)}
	\end{subfigure} \\
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{1} &  \\
			& \gate{T} &  \\
			&  &  \\
			&  & 
		\end{quantikz}
		\caption{Controlled-T with 2 Ancilla}
	\end{subfigure}%
	\begin{subfigure}{0.4\columnwidth}
		\begin{quantikz}
			& \ctrl{3} & \ctrl{1} &  &  & \\
			& \ctrl{2} & \targ{} & \ctrl{2} & \ctrl{1} & \\
			&  &  & \ctrl{1} & \targ{} & \\
			& \targ{} &  & \targ{} &  &
		\end{quantikz}
		\caption{Reversible 1-but full adder}
	\end{subfigure}%
	\caption{4-Qubit unitaries used in the  \cref{tab:SpecificUnitaries}}
	\label{fig:4qubitfigs}
\end{figure}
